Improved Approximations for Vector Bin Packing via Iterative Randomized Rounding

We study the $d$-dimensional Vector Bin Packing ($d$VBP) problem, a generalization of Bin Packing with central applications in resource allocation and scheduling. In $d$VBP, we are given a set of items, each of which is characterized by a $d$-dimensional volume vector; the objective is to partition the items into a minimum number of subsets (bins), such that the total volume of items in each subset is at most $1$ in each dimension. Our main result is an asymptotic approximation algorithm for $d$VBP that yields a ratio of $(1+\ln d-\chi(d) +\varepsilon)$ for all $d \in \mathbb{N}$ and any $\varepsilon > 0$; here, $\chi(d)$ is some strictly positive function. This improves upon the best known asymptotic ratio of $ \left(1+ \ln d +\varepsilon\right)$ due to Bansal, Caprara and Sviridenko (SICOMP 2010) for any $d >3$. By slightly modifying our algorithm to include an initial matching phase and applying a tighter analysis we obtain an asymptotic approximation ratio of $\left(\frac{4}{3}+\varepsilon\right)$ for the special case of $d=2$, thus substantially improving the previous best ratio of $\left(\frac{3}{2}+\varepsilon\right)$ due to Bansal, Elias and Khan (SODA 2016). Our algorithm iteratively solves a configuration LP relaxation for the residual instance (from previous iterations) and samples a small number of configurations based on the solution for the configuration LP. While iterative rounding was already used by Karmarkar and Karp (FOCS 1982) to establish their celebrated result for classic (one-dimensional) Bin Packing, iterative randomized rounding is used here for the first time in the context of (Vector) Bin Packing. Our results show that iterative randomized rounding is a powerful tool for approximating $d$VBP, leading to simple algorithms with improved approximation guarantees.

==> AFPTAS.tex <==
In this section we prove \Cref{lem:AFTPAS}.
Consider an execution of \Cref{alg:basic_round_and_round} on a {\sc Bin Packing} instance $(I,v)$ with $S_0=I$.  Recall that $S_j$ is the set of remaining items after the $j$-th iteration of \Cref{alg:basic_round_and_round}.
The proof hinges on showing that, with high probability, $ \OPT(S_j,v)\lesssim (1-\delta)^{j} \OPT(I,v)$ for any $j\in[k]$ ($k$ is as defined in \Cref{alg:basic_round_and_round}).
To show this property, we utilize a {\em $(1+\eps)$-subset-oblivious} algorithm for {\sc Bin Packing} given by Bansal, Caprara and Sviridenko~\cite{BansalCS2010}.
Subset-oblivious algorithms are a central component in their {\em Round\&Approx} framework~\cite{BansalCS2010}.
Unlike {\em Round\&Approx}, which applies subset-oblivious algorithm to the given instance, in the context of \textsf{Round\&Round} the subset-oblivious algorithm is used only for the analysis, to show the existence of solutions satisfying certain properties.

The following is a slight simplification of the definition of subset-oblivious algorithms by Bansal et al. \cite[Definition 1]{BansalCS2010}.
\begin{defn}
\label{def:afptas_subset_oblivious}
  For $\beta \geq 1$, an algorithm $\appr$
	%$\appr(I,v,S)$ 
  is {\em $\beta$-subset-oblivious} for {\sc Bin Packing} if for any~$\eps>0$ there are $K\in \mathbb{N}$ and $\psi>0$ such that, for any {\sc Bin Packing} instance $(I,v)$, there is a set $\cS\subseteq \mathbb{R}^{I}_{\geq 0}$ of at most $K$ vectors which satisfies the following properties:
  \begin{enumerate}
    \item For any $\bu \in\cS$ it holds that $\tol(\bu)\leq \psi$.
	\item $\OPT(I,v) \geq \max_{\bu \in \cS} \| \bu \|$.
    \item For any $S\subseteq I$, given the  Bin Packing instance $(S,v)$, $\appr$ returns a solution satisfying
	\begin{equation*}
	  \appr(I,v,S)\leq \beta \cdot \max_{\bu \in \cS} \one_S \cdot \bu +\eps \cdot \OPT(I,v) + K,
	\end{equation*}
	where $\appr(I,v,S)$ is the number of bins used by the solution.
  \end{enumerate}
  We refer to $K$ and $\psi$ as the {\em $\eps$-parameters of $\appr$}, and to $\cS$ as the {\em  $\eps$-weight vectors of~$\appr$ and~$(I,v)$}. 
\end{defn}

We use the next result due to Bansal et al.~\cite{BansalCS2010}.
\begin{lemma}
\label{lem:afptas_subset_oblivious}
  For any $\eps>0$ there is a polynomial-time $(1+\eps)$-subset-oblivious algorithm for {\sc Bin Packing}. 
\end{lemma}

Given $\eps>0$, let $(I,v)$ be a {\sc Bin Packing} instance. We assume that $\eps$ and $(I,v)$ are fixed throughout this section.
Also, define $\OPT=\OPT(I,v)$. Consider an execution of \Cref{alg:basic_round_and_round} with $\delta=\min\left\{ \frac{\eps}{200} ,0.05\right\}$, the instance $(I,v)$ and $S_0=I$.
We use $\alpha, k, z_j$ etc. to indicate the respective variables within this execution of the algorithm.
As in \Cref{sec:new_analysis}, we use $(\Omega, \cF,\Pr)$ to denote the probability space generated by the algorithm and assume $\Omega$ is finite.
Similarly, without loss of generality, we  assume that in each iteration $j$, \Cref{alg:basic_round_and_round} samples $\OPT$ configurations  $C^j_1,\ldots, C^j_{\OPT}$ independently according to $\bx^j$, and ignores configurations $C^j_{\rho_j+1},\ldots, C^j_{\OPT}$.
  
Define the random variables  $P_j =(C^j_1,\ldots, C^j_{\OPT})$ for $j = 1,\hdots,k$.
Let $\cF_j = \sigma(P_1,\ldots,P_j)$ be the $\sigma$-algebra of the random variables $P_1,\ldots,P_j$ and $\cF_0 = \{ \emptyset ,\Omega\}$. 
It follows that $\cF_0\subseteq \cF_1 \subseteq \ldots \subseteq \cF_k$.
We note this notation is consistent with the notation used for the probability space in \Cref{sec:new_analysis}, up to the fact that the in this section only \Cref{alg:basic_round_and_round} is used, whereas in \Cref{sec:new_analysis} the probability space refers to an execution of \Cref{alg:match_and_round} which uses \Cref{alg:basic_round_and_round} as a subroutine. 

We use in the analysis the following  variants of lemmas stated in \Cref{sec:new_analysis}. 
\begin{lemma}
\label{lem:AFPTAS_concentration_multistep}
  Let $j\in \{0,1,\ldots, k-1\}$ and $t>0$.
  Also, let $\bu\in \mathbb{R}^I_{\geq 0}$ be an $\cF_{j}$-measurable random vector.
  Then,
  \begin{equation*}
    \Pr\left( \exists r\in \{j,\hdots,k\}:~\bu \cdot \one_{S_{r}} - (1-\delta)^{r-j}\cdot  \bu \cdot \one_{S_j} > t \cdot \tol(\bu) \right) \leq \delta^{-2}\cdot  \exp \left( -\frac{2\cdot\delta^{4} \cdot t^2}{\OPT} \right) \enspace .
  \end{equation*}
\end{lemma}
\begin{lemma}
\label{lem:AFTAS_first_fit_bound}
  With probability at least $1-\delta^{-2}\cdot \exp\left(-\delta^7 \cdot \OPT\right)$, it holds that $\rho^* \leq  16\cdot \delta \cdot \OPT+1$. 
\end{lemma}
The statements and  proofs of \Cref{lem:AFPTAS_concentration_multistep} and \Cref{lem:AFTAS_first_fit_bound} are identical to the statements and proofs of \Cref{lem:concentration_multistep} and \Cref{lem:first_fit_bound}.
The only difference is in the probability spaces to which the lemmas refer.
This is due to the fact that \Cref{alg:basic_round_and_round} is now invoked directly, while previously it was called as a subroutine by~\Cref{alg:match_and_round}.
We therefore omit the proofs.

By \Cref{lem:subset_oblivious}, there is a $(1+\delta^2)$-subset-oblivious algorithm $\appr$ for {\sc Bin Packing}.
Let $K$ and~$\psi$ be its $\delta^2$-parameters, and let $\cS$ be the set of  $\delta^2$-weight vectors of $\appr$ and $(I,v)$.
Observe that by \Cref{def:subset_oblivious}, it holds that $K$ and $\psi$ depend solely on $\delta^2$, and are independent of the instance~$(I,v)$.
Without loss of generality, we assume that $\psi,K>1$. 

\begin{lemma}
\label{lem:AFTPAS_ratio}
  Given $(I,v)$, $S_0=I$ and $\delta$ as defined above, \Cref{alg:basic_round_and_round} returns a solution for $(I,v)$ of size at most $(1+40\delta)\OPT+ 4\delta^{-2}K$ with probability at least $1- 2\cdot K \cdot \delta^{-2} \exp\left( -\frac{2\cdot \delta^8 \cdot  \OPT}{\psi^2}\right)$.
\end{lemma}
\begin{proof}
  We note that the set $\cS$ is non-random, and therefore $\cF_0$-measurable.
  Thus, by \Cref{lem:AFPTAS_concentration_multistep}, for every $\bu\in \cS$ it holds that 
  \begin{equation}
  \label{eq:AFTPAS_concentration}
	\begin{aligned}
	&\Pr\left( \exists j\in \{0,1,\ldots, k\}: \bu\cdot \one_{S_j}>(1-\delta)^j \cdot \| \bu \| +\delta^2 \cdot \OPT\right) \\
	=&\Pr\left( \exists j\in \{0,1,\ldots, k\}: \bu\cdot \one_{S_j}-(1-\delta)^j \cdot \bu \cdot  \one_{S_0} >\frac{\delta^2 \cdot \OPT}{\tol(\bu)}\cdot \tol(\bu) \right)\\
	\leq& \delta^{-2}\cdot\exp  \left( -\frac{2\cdot \delta^4\cdot \left( \frac{\delta^2 \cdot \OPT}{\tol(\bu)}\right)^2 }{\OPT}\right)\\
	\leq & \delta^{-2} \cdot \exp\left( -\frac{2\cdot \delta^8 \cdot \OPT}{\psi^2}\right),
    \end{aligned}
  \end{equation}
  where the last inequality uses $\tol(\bu)\leq \psi$.
  As $|\cS|\leq K$, we can use \eqref{eq:AFTPAS_concentration} and the union bound to get
  \begin{equation}
  \label{eq:AFTPAS_concentration_combined}
    \begin{aligned}
      &\Pr\left( \exists \bu \in \cS ,~ j\in \{0,1,\ldots, k\}: \bu\cdot \one_{S_j}>(1-\delta)^j  \| \bu \| +\delta^2  \OPT\right) \leq K \delta^{-2} \exp\left( -\frac{2 \delta^8  \OPT}{\psi^2}\right)\enspace.
    \end{aligned}
  \end{equation}
  For the remainder of the proof we assume that 
  \begin{equation}
  \label{eq:AFTPAS_first_assumption}
    \forall  j\in \{0,1,\ldots, k\}, ~\bu\in \cS: ~~~\bu\cdot \one_{S_j}\leq(1-\delta)^j  \| \bu \| +\delta^2  \OPT\enspace.
  \end{equation}
  By \eqref{eq:AFTPAS_concentration_combined}, this assumption holds with probability at least  $1-K\cdot  \delta^{-2}\cdot  \exp\left( -\frac{2\cdot \delta^8 \cdot  \OPT}{\psi^2}\right)$. 
  
  Recall that $\OPT(I,v)\geq \max_{\bu\in \cS} \|\bu\|$ (\Cref{def:subset_oblivious}).
  Thus,
  \begin{equation}
  	\label{eq:AFPTAS_uniform_bound}
  \forall  j\in \{0,1,\ldots, k\}, ~\bu\in \cS: ~~~\bu\cdot \one_{S_j}\leq (1-\delta)^j  \| \bu \| +\delta^2  \OPT\leq (1-\delta)^{j}\cdot \OPT+\delta^2\dot \OPT,
  \end{equation}
  where the first inequality is by \eqref{eq:AFTPAS_first_assumption}. Hence, by \Cref{def:subset_oblivious}, for every $j=1,\ldots, k$ it holds that
  \begin{equation}
  \label{eq:AFTPAS_appr_bound}
    \begin{aligned}
	\appr(I,v,S_{j-1})&\leq (1+\delta^2)\cdot  \max_{\bu \in \cS} \one_{S_{j-1}} \cdot \bu +\delta^2 \cdot \OPT +K \\
	&\leq (1+\delta^2)\cdot \left( (1-\delta)^{j-1}\cdot \OPT+\delta^2\dot \OPT \right)  +\delta^2 \cdot\OPT +K\\
	&\leq (1+\delta^2)\cdot (1-\delta)^{j-1}\cdot \OPT +3\cdot \delta^2 \cdot\OPT +K,
    \end{aligned} 
  \end{equation}
  where the second inequality is by \eqref{eq:AFPTAS_uniform_bound}. 
	
  Recall that $\OPT_f(\bd)$ is the value of an optimal solution of \eqref{eq:config_LP}. 
  Since $\appr$
	% $\appr(I,v,S_j)$ 
  returns a solution for $(S_j,v)$, it follows that $\OPT_f(\one_{S_j})\leq\OPT(S_j,v)\leq \appr(I,v,S_j)$.
  Since \Cref{round:LPS} of \Cref{alg:basic_round_and_round}  finds a $(1+\delta^2)$-approximate solution for $\LP(\one_{S_{j-1}})$  it follows that $z_j \leq (1+\delta^2) \cdot \OPT_f(\one_{S_{j-1}}) \leq (1+\delta^2)\cdot \appr(I,v,S_{j-1} )$. Using this observation  and \eqref{eq:AFTPAS_appr_bound}, we have
  \begin{equation*}
	\begin{aligned}
	z_j &\leq (1+\delta)^2\cdot \appr(I,v,S_{j-1} )\\
	&\leq (1+\delta^2)\cdot \left( (1+\delta^2)\cdot (1-\delta)^{j-1}\cdot \OPT +3\cdot \delta^2 \cdot\OPT +K\right)\\
	&\leq  (1+4\delta^2) \cdot (1-\delta)^{j-1}\cdot \OPT +4\cdot \delta^2 \cdot\OPT+2\cdot K\enspace.
	\end{aligned}
  \end{equation*}
  Hence,
  \begin{equation}
  \label{eq:AFPTAS_z_sum}
    \begin{aligned}
	\delta \cdot \sum_{j=1}^{k} z_j & \leq\delta \cdot\sum_{j=1}^{k} \left(   (1+4\delta^2) \cdot (1-\delta)^{j-1}\cdot \OPT +4\cdot \delta^2 \cdot\OPT +2\cdot K \right) \\
	&\leq \delta \cdot (1+4\delta^2)\cdot  \frac{1-(1-\delta)^{k} }{1-(1-\delta) }\cdot\OPT + k\cdot4\cdot  \delta^3 \cdot \OPT+2\delta\cdot k \cdot  K  \\
	&\leq  (1+4\delta^2)\cdot \OPT +4\delta\cdot\OPT +2\delta^{-1}\cdot K,
	\end{aligned}
  \end{equation}
  where the last inequality uses $k\leq \delta^{-2}$. 
	
  Recall the algorithm samples $\rho_j=\ceil{\alpha \cdot z_j}$ configurations in each iteration.
  Thus,
  \begin{equation}
    \label{eq:AFPTAS_rho_bound}
	\begin{aligned}
		\sum_{j=1}^{k} \rho_j &=\sum_{j=1}^{k} \ceil{\alpha \cdot z_j}\\
		&\leq \delta^{-2} + (1+\delta)\cdot \delta \cdot \sum_{j=1}^{k} z_j\\
		&\leq \delta^{-2} +(1+\delta )\cdot \left((1+4\delta^2)\cdot \OPT +4\delta\cdot\OPT +2\delta^{-1}\cdot K\right)\\
		&\leq (1+20\delta)\cdot \OPT +2\cdot  \delta^{-2}\cdot K.
		\end{aligned}
  \end{equation}
  The first inequality uses $\alpha\leq \delta \cdot(1+\delta)$ and $k\leq \delta^{-2}$.
  The second inequality is by \eqref{eq:AFPTAS_z_sum}.

  Assume that
  \begin{equation}
  \label{eq:AFPTAS_second_assumption}
    \rho^*\leq 16\cdot\delta \OPT +1 \enspace .
  \end{equation}
  By \Cref{lem:AFTAS_first_fit_bound}, this assumption holds with probability at least $1-\delta^{-2}\cdot \exp(-\delta^{-7}\cdot \OPT)$. Let $m$ be the size of the solution returned by the algorithm.
  Then,
  \begin{equation}
    \label{eq:AFTPAS_m_bound}
	m= \rho^*+ \sum_{j=1}^{k}\rho_j \leq  16\cdot\delta \OPT +1+(1+20\delta)\cdot \OPT +2\cdot \delta^{-2}\cdot K\leq (1+40\delta)\OPT+ 4\delta^{-2}K,
  \end{equation}
  where the first inequality holds by \eqref{eq:AFPTAS_rho_bound} and \eqref{eq:AFPTAS_second_assumption}.
  As we assumed \eqref{eq:AFTPAS_first_assumption} and \eqref{eq:AFPTAS_second_assumption} hold, it follows that~\eqref{eq:AFTPAS_m_bound} holds with probability at least 
  \begin{equation*}
    1-K\cdot  \delta^{-2}\cdot  \exp\left( -\frac{2\cdot \delta^8 \cdot \OPT}{\psi^2}\right)-\delta^{-2}\cdot \exp(-\delta^{-7}\cdot \OPT) \geq 1- 2\cdot K \cdot \delta^{-2} \exp\left( -\frac{2\cdot \delta^8 \cdot  \OPT}{\psi^2}\right)\enspace .
  \end{equation*}
\end{proof} 

Observe that $4\cdot \delta^{-2}\cdot K = o(\OPT)$, and $ \left( 1- 2\cdot K \cdot \delta^{-2} \cdot \exp\left(-\frac{2\cdot\delta^2\cdot \OPT}{\psi^2} \right)\right)\xrightarrow[\OPT\rightarrow \infty]{}1$.
Hence, the next result follows immediately from~\Cref{lem:AFTPAS_ratio}.
\begin{cor}
\label{cor:AFTPAS}
  For any $\eps>0$, \Cref{alg:basic_round_and_round} is a randomized asymptotic $(1+\eps)$-approximation for {\sc Bin Packing} when invoked with $\delta=\min\left\{\frac{\eps}{200}, 0.05\right\}$.
\end{cor}

\begin{proof}[{\bf Proof of \Cref{lem:AFTPAS}}]
  It is well-known that \eqref{eq:config_LP} admits an FPTAS for {\sc Bin Packing} instances and vectors $\bd\in \{0,1\}^{I}$.
  Indeed, in this case the separation oracle for the dual of \eqref{eq:config_LP} needs to solve an instance of the (standard) {\sc Knapsack} problem, for which there is an FPTAS (see, e.g., \cite{Vazirani2001}).
  Hence, the run time of each iteration in \Cref{round:loop} of \Cref{alg:basic_round_and_round} (given a {\sc Bin Packing} instance) is polynomial in the instance size and in $\delta^{-2}$.
  As the number of iterations is $k\leq \delta^{-2}$, it follows that the total run time is polynomial in the input size and in $\frac{1}{\delta}$.
  Thus, using~\Cref{cor:AFTPAS}, we have that~\Cref{alg:basic_round_and_round} is a randomized AFPTAS for {\sc Bin Packing}. 
\end{proof} 
